Synthetic Homotopy Theory

The goal of this dissertation is to present results from synthetic homotopy theory based on homotopy type theory (HoTT). After an introduction to Martin-L\"of's dependent type theory and homotopy type theory, key results include a synthetic construction of the Hopf fibration, a proof of the Blakers--Massey theorem, and a derivation of the Freudenthal suspension theorem, with calculations of some homotopy groups of $n$-spheres.

==> temp <==
@(hott|brunerie|blakers|pinsn|kbh|hott-agda|rijke|martin|higher|aw|semantics|cayley|rpn|les-group|syn-coho|syn-ho|cellular|rezk|anel|hatcher)(\{\[\}(.*)\{\]\})?


\\protect\{\\cite\{(.*?)\}\}\{\[\}(.*?)\{\]\}
